Revisiting Transmission Scheduling in RF Energy Harvesting Wireless Communications

The transmission scheduling is a critical problem in radio frequency (RF) energy harvesting communications. Existing transmission strategies in an RF-based energy harvesting system is mainly based on a classic model, in which the data transmission is scheduled in a fixed feasible energy tunnel. In this paper, we re-examine the classic energy harvesting model and show through the theoretical analysis and experimental results that the bounds of feasible energy tunnel are dynamic, which can be affected by the transmission scheduling due to the impact of residual energy on the harvested one. To describe a practical energy harvesting process more accurately, a new model is proposed by adding a feedback loop that reflects the interplay between the energy harvest and the data transmission. Furthermore, to improve network performance, we revisit the design of an optimal transmission scheduling strategy based on the new model. To handle the challenge of the endless feedback loop in the new model, a recursive algorithm is developed. The simulation results reveal that the new transmission scheduling strategy can balance the efficiency of energy reception and energy utilization regardless of the length of energy packets, achieving improved throughput performance for wireless communications.

==> OnTranStr.tex <==
\section{Online Suboptimal Strategy}
\label{sec:onopt}
Although the optimal transmission power in the current epoch is determined by each energy packet arrived in the past and future, their impacts, however, are not equivalent. In particular, a nearby energy packet causes much heavier impact on the current transmission strategy than a remote one. Therefore, if an EHD can predict the length and the arrival time of energy packets that will be received in a near future, an online strategy with near optimal performance can be expected.

Now, recall that the harvested energy reaches the global maximum when the EHD maintains a specific amount of residual energy as specified in (\ref{eq:4_08}).
One possible transmission strategy is to maximize the energy harvested from each energy packet. Compared with the conventional transmission strategy presented in~\cite{tutuncuoglu2012optimum}, which is denoted by $\texttt{ST}_\texttt{2}$, that aims at optimizing the utilization of energy stored in the battery, $\texttt{ST}_\texttt{1}$ maximizes the efficiency of an energy harvesting process. 

Actually, neither $\texttt{ST}_\texttt{1}$ nor $\texttt{ST}_\texttt{2}$ is an optimal solution to improve an EHD's throughput, since a most efficient transmission strategy, which is denoted by $\texttt{ST}_\texttt{0}$, needs to balance the efficiencies of energy harvest and energy utilization. Nevertheless,  the simulation results of Figure~\ref{fig:perfcmp_thr_tau}, which will be presented in Section~\ref{subsec:perEva_onOff},  demonstrate the following two critical observations:

\begin{obser}
\label{obser:01}
	\emph\emph{{If the average length of energy packets is not much shorter than the time constant of a charging circuit, the optimal transmission strategy approaches the maximum energy harvesting one, i.e.,  $\texttt{ST}_\texttt{0}\to\texttt{ST}_\texttt{1}$, if  $\bar{T}^e\!\not\ll\!\tau$.}}
\end{obser}

\begin{obser}
\label{obser:02}
	\emph\emph{{If the average length of energy packets is much shorter than the time constant of a charging circuit, the optimal transmission strategy  approaches the conventional one, i.e., $\texttt{ST}_\texttt{0}\to\texttt{ST}_\texttt{2}$, if  $\bar{T}^e\!\ll\!\tau$.}}
\end{obser}

The strategy $\texttt{ST}_\texttt{2}$ is based on the classic model and a state-of-the-art of its online solutions can be found in \cite{ulukus2015energy}. Therefore, we focus on the scenario of Observation~\ref{newpro:01}, where $\bar{T}^e\!\not\ll\!\tau$. The development of an online strategy in such a scenario can be classified into following two cases:
\vspace{0.1cm}
\begin{adjustwidth}{-0.32cm}{-0.3cm}
\begin{itemize}
  \item[\textendash] \emph{Correlated harvesting process:} If an EHD is powered by a dedicated energy source, e.g.,  RF identification (RFID) system, the length and arrival time of neighboring energy packets are usually highly correlated~\cite{das2014rfid, kaur2011rfid}. 
  \item[\textendash] \emph{Uncorrelated harvesting process:} If an EHD harvests energy from ambient RF signals radiated from multiple sources, the length and the time that an energy packet arrives at the EHD are random. 
\end{itemize}
\end{adjustwidth}
\vspace{0.1cm}

In the first case, the prediction model, such as a Markov chain and an adaptive filter~\cite{michelusi2013transmission}, can be applied to estimate the length and the arrival time of incoming energy packet. To be specific, after receiving the $i^{th}$ energy packet at $t_i$, the EHD predicts the length and arrival time of the incoming energy packet, which is denoted by $\hat{T}^e_{i+1}$ and $\hat{t}_{i+1}$, respectively. Later on, substituting $\hat{T}^e_{i+1}$ into (\ref{eq:7_01}) to estimate the residual energy, which is denoted by $\hat{E}^r_{i+1}$,  that needs to be retained in the capacitor before the next epoch. Afterward, the transmission power at epoch $i$, which is denoted by $\hat{p}_i$, can be calculated as follows:
 \begin{equation}\label{eq:7_02}
   \hat{p}_i= \left\{
    \begin{array}{lll}
        \vspace{0cm}
        \displaystyle\frac{E^r_i+E^h_i-\hat{E}^r_{i+1}}{\hat{t}_{i+1}-t_i}, \quad &E^r_i+E^h_i> \hat{E}^r_{i+1},\\
        \vspace{0cm}
        0, \quad &\mathrm{otherwise}.\\
    \end{array}
    \right.
\end{equation}
In the second case, an EHD estimates the residual energy before the next epoch through the average length and time interval of past energy packets, and then determines its current transmission power based on (\ref{eq:7_02}).













